Leveraging ASIC AI Chips for Homomorphic Encryption

Homomorphic Encryption (HE) provides strong data privacy for cloud services but at the cost of prohibitive computational overhead. While GPUs have emerged as a practical platform for accelerating HE, there remains an order-of-magnitude energy-efficiency gap compared to specialized (but expensive) HE ASICs. This paper explores an alternate direction: leveraging existing AI accelerators, like Google's TPUs with coarse-grained compute and memory architectures, to offer a path toward ASIC-level energy efficiency for HE. However, this architectural paradigm creates a fundamental mismatch with SoTA HE algorithms designed for GPUs. These algorithms rely heavily on: (1) high-precision (32-bit) integer arithmetic to now run on a TPU's low-throughput vector unit, leaving its high-throughput low-precision (8-bit) matrix engine (MXU) idle, and (2) fine-grained data permutations that are inefficient on the TPU's coarse-grained memory subsystem. Consequently, porting GPU-optimized HE libraries to TPUs results in severe resource under-utilization and performance degradation. To tackle above challenges, we introduce CROSS, a compiler framework that systematically transforms HE workloads to align with the TPU's architecture. CROSS makes two key contributions: (1) Basis-Aligned Transformation (BAT), a novel technique that converts high-precision modular arithmetic into dense, low-precision (INT8) matrix multiplications, unlocking and improving the utilization of TPU's MXU for HE, and (2) Memory-Aligned Transformation (MAT), which eliminates costly runtime data reordering by embedding reordering into compute kernels through offline parameter transformation. CROSS (TPU v6e) achieves higher throughput per watt on NTT and HE operators than WarpDrive, FIDESlib, FAB, HEAP, and Cheddar, establishing AI ASIC as the SotA efficient platform for HE operators. Code: https://github.com/EfficientPPML/CROSS

==> src/11-BAT_Reduction.tex <==

\subsection{Upgraded BAT Lazy}
1. Split each partial sum:
\begin{align} & psum_j \\ 
&= \underbrace{(psum_j \bmod 2^{8(K-j)})}{L_j} + \underbrace{\lfloor psum_j / 2^{8(K-j)} \rfloor}{H_j} \times 2^{8(K-j)} 
\end{align}

2. Substitute and Rearrange: Substituting this back into the main equation:
\begin{align} & z\\ 
&= \left( \sum_{j=0}^{K-1} \left( L_j + H_j \times 2^{8(K-j)} \right) \times 2^{8j} \right) \bmod q \\ 
&= \left( \sum_{j=0}^{K-1} \left( L_j \times 2^{8j} + H_j \times 2^{8K} \right) \right) \bmod q \\
&= \left( \underbrace{\sum_{j=0}^{K-1} L_j \times 2^{8j}}_{\text{Accumulate Low $K$ bytes}} + \left( \underbrace{\sum{j=0}^{K-1} H_j}_{\text{Accumulate High $K$ bytes}} \right) \times 2^{8K} \right) \bmod q 
\end{align}

3. Apply Modular Reduction to High Part:
\begin{align} & \text{Reduction Term} \\ 
&= \left( \sum_{k} s_k 2^{8k} \right) \times 2^{8K} \bmod q \\ 
&= \sum_{k} s_k \times (2^{8(K+k)} \bmod q) \\ 
&= \sum_{k} s_k \times \left( \sum_{l=0}^{K-1} R_{k,l} \times 2^{8l} \right) \quad \text{(using matrix } R) 
\end{align}
% & =\left(  \sum_{j=0}^{j=K-1} (psum_j \times 2^{8j}) \bmod q  \right)\bmod q

% \begin{algorithm}
% \caption{\RevA{High-Precise MatMul using BAT.}} \label{alg:bat_deployment}
% \begin{algorithmic}[1]
% \Require modulus $q$; $A\in\mathbb{Z}_q^{H\times V}$; base $\beta=2^{bp}$; $K=\lceil\log_\beta q\rceil=\lceil \frac{\log q}{bp}\rceil$, indicating number of bytes; $B\in\mathbb{Z}_q^{V\times W}$; hardware supports $bp$-bit arithmetic. %This algorithm is provided only for illustration to contrast BAT with SoTA GPU designs. Refer to \algref{} for the production-grade, faster BAT algorithm.
% \item[]
% \item[]
% \hspace{-2em} \textbf{\textsc{ChunkDecompose}}{($a$)}{}$\rightarrow \left[a^{k}\right]_{0\le k < K}$
% % \State  \textit{\textbf{--\hfill ChunkDecomposition$(a)$  $\rightarrow \left( a^{k}, k \in \left[0, \lceil \frac{logq}{bp}\rceil -1 \right] \right)$ \hfill--}}  
% % \State  $a^{k}\leftarrow $ bit range $\left[k\cdot bp, (k\+1)\cdot bp \right]$ of $a$, $0 \leq k < \lceil \frac{logq}{bp} \rceil$
% \State \textbf{for} $k = 0$ \textbf{to} $K-1$:
% \State \quad  $a^{k}\leftarrow $ $a\left[k\cdot bp: (k+1)\cdot bp \right]$ \hfill $\triangleright$ Select $k$-th $bp$ bits of $a$. 
% \State \textbf{Return} $\left[a^{k}\right]_{0\le k < K}$
% \item[]
% \item[]
% \hspace{-2em} \textbf{\textsc{ChunkDecomposeRightMatrix}}{($a$)}{}$\rightarrow \left[a^{k}\right]_{0\le k < K}$ \hfill $\triangleright$ Left Matrix in \figref{fig:ModMatMul}.
% \State \textbf{for} $h=0..H-1$
% \State \quad \textbf{for} $v=0..V-1$
% \State \quad \quad  $\left[a_{h,v}^{k}\right]_{0\le k < K}=\sum_{j=0}^{K-1} a_{h,v}^{(j)}\beta^j$
% \State \quad \quad \textbf{for} $i=0$ \textbf{to} $K$
% \State \quad \quad \quad \textbf{for} $j=0..K-1$
% \State \quad \quad \quad \quad $A'_{Kh+i,\ Kv+j}\leftarrow a_{h,v}^{(j)}\cdot\beta^i \bmod q$
% \State \textbf{Return} $A'$
% \item[]
% \item[]
% \hspace{-2em} \RevA{\textbf{\textsc{BAT\_RightMatrix}}{($X, bp, q$)}{} $\rightarrow X$} \hfill $\triangleright$ Left Matrix in \figref{fig:ModMatMul}.
% \State \textbf{for} $v=0$ \textbf{ to }$V-1$
% \State \quad \textbf{for} $w=0$ \textbf{ to } $W-1$
% \State \quad \quad Decompose $b_{v,w}=\sum_{j=0}^{K-1} b_{v,w}^{(j)}\beta^j$\;
% \State {$j=0..K-1$}{
%       $B'_{Kv+j,\ w}\leftarrow b_{v,w}^{(j)}$\;
%     }

% \item[]
% \item[]
% \hspace{-2em} \textbf{\textsc{Main-HPScalarMult}}{($a, b$)} $\rightarrow z$ 
% \State $\left[\hat{a}^k_i\right]_{0\le i,k < K} \leftarrow$ \Call{OfflineCompile}{$a$} \hfill $\triangleright$ \ding{185} in \figref{fig:ModMatMul}.
% \State $\left[b^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$b$}
% \State $\left[psum^{k}\right]$ = $\left[\hat{a}^k_i\right] \times \left[b^k\right]$, $0 \le i,k < K$
% \State \textbf{for} $k=0$ \textbf{to} $K-1$:
% \State \quad $z \mathrel{+}= psum^{k} \ll (bp*k)$ \hfill $\triangleright$ \ding{186} in \figref{fig:CROSS_Scalar_Flow}.
% \State \textbf{Return} $z$
% \end{algorithmic}
% \end{algorithm}

\subsection{BAT for Modular Reduction}

% \begin{algorithm}
% \caption{BAT Lazy Reduction $r = x \bmod q$}
% \label{alg:lazy_red}

% \begin{algorithmic}[1]

% \Require Integer $x$ (to reduce), modulus $q$ 

% \State $L=\lceil \log_{256}(q) \rceil$  \hfill  $\triangleright$ {Number of bytes to represent $q$}
% \State $x = \sum_{i=0}^{2L+3} x[8i+7: 8i] \cdot 256^{i}$ $\triangleright$ {$x[8i+7: 8i]$: bytes of $x$}
% \State $A=\sum_{i=0}^{L-1} x[8i+7: 8i] \cdot 256^{i}$ $\triangleright$ {Lower $L$ bytes, not reduced}

% \hspace{-12mm} \texttt{BAT Lazy Reduction Algorithm}

% \State Initialize: $\text{out} = A$
% \State \textbf{for} {$i = L$ \textbf{to} $2L+3$}  \hfill $\triangleright$ {Higher $L$ Bytes, Reduce $B$}
% \State \quad $\text{out} = \text{out} + x[8i+7: 8i] \cdot 256^i \bmod q$
% \State \textbf{Return} $\text{out}$ \hfill $\triangleright$ {$L+2$ Bytes, Partially Reduced}

% \hspace{-12mm} \texttt{Implementation of BAT Lazy Red.}

% \hspace{-12mm} \texttt{Offline} \hfill $\triangleright$ {Precompute Reduction Coefficients}
% \State $r_i = 256^{i+L} \bmod q, i\in[0,L+3]$ \hfill 
% \State $R_{i,j} = r_i[8j+7:8j], j\in[0,L-1]$ \hfill 

% \hspace{-12mm} \texttt{Online} \hfill $\triangleright$ {Reduce High Part for a Batch of $b$ values}
% \State $B_{idx,i}=x_{idx}[8i+7:8i], idx\in[0,b-1], i\in[L,2L+3]$
% \State return $B_{idx,i}@R_{i,j} + A_{idx,j} $ \hfill $\triangleright$ {uint8 $b\cdot(L+4)\cdot L$ MatMul}

% \end{algorithmic}
% \end{algorithm}

% \subsubsection{Byte-form Representation}
\label{sec:correct_slice}

\eqref{eq:line10} generates result: % \ding{382} in \figref{fig:CROSS_Scalar_Flow} produces partial sum of 18 bits, written as $psum_j$, where $i\in[0,3]$, the final reduction needs to bring it back within 32 bits. 

% To implement lazy reduction effectively with TPU's low-precision arithmetic, \framework represents high-precision values as vectors of 8-bit ``digits". Given modulus $q$ requires $L$ bytes, any intermediate result $x$ up to $2L+4$ bytes can be represented as:
\begin{comment} % Good try but fail.
\begin{align}
% & \text{\eqref{eq:line10}} \\
& = \sum \left( \underbrace{\begin{bmatrix}
psum_{0} \\
psum_{1} \\
\vdots \\
psum_{K-1}
\end{bmatrix}}_{16+log_2(K)\text{ bits each}} \times \ \ \begin{bmatrix}
2^0 \\
2^8  \\
\vdots \\
2^{8(K-1)} 
\end{bmatrix} \right) \bmod q \label{eq:line11}
\\
& = \left( \sum_{j=0}^{j=K-1} ( \underbrace{psum_j}_{16+log_2(K)\ \text{bits}} \times 2^{8j} ) \right) \bmod q \\
& =\left(  \sum_{j=0}^{j=K-1} (psum_j \times 2^{8j}) \bmod q  \right)\bmod q \\
& =\left(  \sum_{j=0}^{j=K-1}  psum_j \times \underbrace{\left(2^{8j} \bmod q  \right)}_{computed\ offline\ as\ LC_j}  \right)\bmod q \\
& =\left(  \sum_{j=0}^{j=K-1}  \underbrace{psum_j}_{16+log_2(K)\ \text{bits}} \times \underbrace{LC_j}_{K\ \text{bytes}}  \right) \underbrace{\bmod q}_{delay\ till\ final} \\
& = \sum_{j=0}^{j=K-1}  \left( \underbrace{psum_j}_{16+log_2(K)\ \text{bits}} \times  \sum_{k=0}^{k=K-1} (\underbrace{ LC_{j,k}}_{\text{one byte each}}\times 2^{8k}) \right) \bmod q  \\
& = \left( \sum_{k=0}^{k=K-1} \left(\sum_{j=0}^{j=K-1} {psum_j} \times  LC_{j,k}\right) \times 2^{8k} \right) \bmod q  \\
& = \sum \left( 
\underbrace{\begin{bmatrix}
psum_{0} \\
psum_{1} \\
\vdots \\
psum_{K-1}
\end{bmatrix}}_{16+log_2(K) \text{ bits}} \times 
\underbrace{\begin{bmatrix}
LC_{0,0}  & \cdots & LC_{0,K-1} \\
LC_{1,0}  & \cdots & LC_{1,K-1} \\
\vdots        & \ddots & \vdots        \\
LC_{K-1,0} & \cdots & LC_{K-1,K-1}
\end{bmatrix}}_{ K\times K \text{ 8-bit matrix}} \times\begin{bmatrix}
2^0 \\
2^8  \\
\vdots \\
2^{8(K-1)} 
\end{bmatrix} \right) \bmod q \label{eq:line10}
\end{align}
\end{comment}

% \begin{align}
% & =\left(  \sum_{j=0}^{j=2K-1} (c_j \times 2^{8j}) \right)\bmod q \\
% & =\left( \sum_{j=K}^{j=2K-1} (c_j \times \underbrace{(2^{8j} \bmod q)}_{\text{compute offline as } LC_j}) + \sum_{j=0}^{j=K-1} (c_j \times 2^{8j}) \right)\bmod q \\
% & =\left( \underbrace{\sum_{j=K}^{j=2K-1} (c_j \times 2^{8j})}_{\text{Need to be reduced}} + \underbrace{c \land (2^{8(K-1)}-1)}_{\text{low $K$ bytes}}  \right)\bmod q \\
% & =\left( \sum_{j=K}^{j=2K-1} (c_j \times \underbrace{(2^{8j} \bmod q)}_{\text{compute offline as } LC_j}) + \underbrace{c \land (2^{8(K-1)}-1)}_{\text{low $K$ bytes}} \right)\bmod q \\
% & =\left( \sum_{j=K}^{j=2K-1} (c_j \times \underbrace{LC_j}_{K\text{ Bytes}}) + \sum_{j=0}^{j=K-1} (c_j \times 2^{8j}) \right)\bmod q \\
% & = \sum_{j=0}^{j=K-1}  \left( \underbrace{psum_j}_{16+log_2(K)\ \text{bits}} \times  \sum_{k=0}^{k=K-1} (\underbrace{ LC_{j,k}}_{\text{one byte each}}\times 2^{8k}) \right) \bmod q  \\
% & = \left( \sum_{k=0}^{k=K-1} \left(\sum_{j=0}^{j=K-1} {psum_j} \times  LC_{j,k}\right) \times 2^{8k} \right) \bmod q  \\
% & = \sum \left( 
% \underbrace{\begin{bmatrix}
% psum_{0} \\
% psum_{1} \\
% \vdots \\
% psum_{K-1}
% \end{bmatrix}}_{16+log_2(K) \text{ bits}} \times 
% \underbrace{\begin{bmatrix}
% LC_{0,0}  & \cdots & LC_{0,K-1} \\
% LC_{1,0}  & \cdots & LC_{1,K-1} \\
% \vdots        & \ddots & \vdots        \\
% LC_{K-1,0} & \cdots & LC_{K-1,K-1}
% \end{bmatrix}}_{ K\times K \text{ 8-bit matrix}} \times\begin{bmatrix}
% 2^0 \\
% 2^8  \\
% \vdots \\
% 2^{8(K-1)} 
% \end{bmatrix} \right) \bmod q 
% \end{align}
\begin{align} 
& =\left( \sum_{j=0}^{j=2K-1} (c_j \times 2^{8j}) \right)\bmod q \\ 
& =\left( \sum_{j=K}^{j=2K-1} (c_j \times \underbrace{(2^{8j} \bmod q)}_{\text{compute offline as } LC_j}) + \sum_{j=0}^{j=K-1} (c_j \times 2^{8j}) \right)\bmod q \\ 
& =\left( \sum_{j=K}^{j=2K-1} \left( c_j \times \sum_{l=0}^{K-1} (R_{j-K, l} \times 2^{8l}) \right) + \sum_{l=0}^{K-1} (c_l \times 2^{8l}) \right)\bmod q \\  & \quad \text{ (where } R_{j-K, l} \text{ is the } l\text{-th byte of } LC_j, \text{ stored in } \texttt{self.R} \text{)} \nonumber \\  
& =\left( \sum_{l=0}^{K-1} 2^{8l} \left( \underbrace{c_l}_{\text{Lower $K$ bytes}} + \sum_{j=K}^{2K-1} (c_j \times R_{j-K, l}) \right) \right)\bmod q \\  
% & =\left( \sum_{l=0}^{K-1} 2^{8l} \left( A_l + \underbrace{\sum_{k=0}^{K-1} (B_k \times R_{k, l})}_{\text{Matrix Mul } B \times R} \right) \right)\bmod q \end{align}
% \begin{align}  
& =\left( \sum_{l=0}^{K-1} 2^{8l} \left( c_l + \sum_{j=K}^{2K-1} (c_j \times R_{j-K, l}) \right) \right)\bmod q \\ 
& \quad \text{Let } k = j - K \text{ (change of variable for the inner sum)} \nonumber \\ 
& \quad \text{Then } j = k + K, \text{ and the range } [K, 2K-1] \text{ becomes } [0, K-1] \nonumber \\ 
& =\left( \sum_{l=0}^{K-1} 2^{8l} \left( c_l + \sum_{k=0}^{K-1} (c_{k+K} \times R_{k, l}) \right) \right)\bmod q \\ 
& \quad \text{Define components } A \text{ and } B \text{ (splitting input } c \text{):} \nonumber \\ 
& \quad A_l = c_l \quad (\text{Lower bytes, } 0 \le l < K) \nonumber \\ 
& \quad B_k = c_{k+K} \quad (\text{Higher bytes, } 0 \le k < K) \nonumber \\ 
& =\left( \sum_{l=0}^{K-1} 2^{8l} \left( A_l + \sum_{k=0}^{K-1} (B_k \times R_{k, l}) \right) \right)\bmod q \\ 
& \quad \text{Recognize the matrix-vector product } (B \times R)l = \sum{k} B_k R_{k,l} \nonumber \\ 
& =\left( \sum_{l=0}^{K-1} 2^{8l} \left( A_l + (B \times R)_l \right) \right)\bmod q 
\end{align}

% \subsection{Detailed TPU Setup for NTT Throughput}
% \label{sec:tpu_setup_for_NTT_throughput}
% \textbf{TPU Setup}: We use a single full-host TPU virtual machine as the underlying device, as shown in \tabref{tab:ntt_throughput_setup}. We observes that TPU scales super-linearly (better than linear scaling) in our test cases when sharding batch dimension across TPU instances. Different tensor core achieves the nearly same latency under sharding setup. Therefore, we report latency of a single Tensor Core in other experiment to reflect critical path latency.%For fairness of throughput comparison, we scale TPU instances to roughly similar power as NVIDIA A100 used in TensorFHE\cite{fan2022tensorfhe} as shown in \tabref{tab:ntt_throughput_setup}. In all these setup, JAX shows the same number of four devices for all these four generations of TPUs.

% \textbf{Security Parameter Setup}: \compiler implements the Set A,B,C in \tabref{tab:ntt_throughput} with 28-bit moduli (\tabref{tab:ntt_throughput_setup}).

% \begin{table}[!htp]\centering
% \caption{Evaluation Setup for NTT Throughput Comparison. The GFLOPs, bandwidth of HBM and VMEM Read and Write are obtained from Xprof profiling for \textbf{one tensor core}.}\label{tab:ntt_throughput_setup}
% \resizebox{\columnwidth}{!}{ % use this if the table is too large
% \begin{tabular}{cccccc}\hline
% Hardware &\textbf{TPUv4} &\textbf{TPUv5e} &\textbf{TPUv6e} &\textbf{TPUv5p} \\\hline
% \# JAX Logical Devices & 8 & 16 & 16 & 8 \\
% Setup &v4-16 &v5litepod-16 &v6e-16 &v5-16 \\
% \# Tensor Cores & 16 & 16 & 16 & 16 \\ \hline
% GFLOPs &139800 &202700 &918000 &236700 \\
% HBM BW (GiB/s) &572.2 &762.9 &1525.5 &1287.45 \\
% VMEM Read BW (GiB/s) &2003 &17166.1 &21696.1 &20027.2 \\
% VMEM Write BW (GiB/s) &1001 &5722.05 &15020.4 &6675.72 \\\hline\hline
%  & &\textbf{Set A} &\textbf{Set B} &\textbf{Set C} \\\hline
% \multirow{4}{*}{\makecell{Security \\ Configuration}} &Q &109 &218 &438 \\
% &Degree &$2^{12}$ &$2^{13}$ &$2^{14}$ \\
% &$log_2(q)$ &28 &28 &28 \\
% &\# Limbs &4 &8 &15 \\
% \hline
% \end{tabular}}
% TPUv6e offers higher GFLOPs as its takes 256$\times$256 systolic array.
% \end{table}

 %We mainly provide results on TPUv4 as it's freely available at TPU research cloud.


% \begin{algorithm}
% \caption{Tensor Lazy Reduction $r = x \bmod q$}
% \label{alg:lazy_red}
% \begin{algorithmic}[1]
% \Require Integer $x$ (to reduce), modulus $q$ 
% \State $L=\lceil \log_{256}(q) \rceil$  \hfill  $\triangleright$ Number of bytes to represent $q$
% \State $x = \sum_{i=0}^{2L+3} x[8i+7: 8i] \cdot 256^{i}$ \hfill $\triangleright$  $x[8i+7: 8i]$: bytes of $x$
% \State $A=\sum_{i=0}^{L-1} x[8i+7: 8i] \cdot 256^{i}$   \hfill $\triangleright$ Lower $L$ bytes, not reduced

% \hfill 

% \noindent \hspace{-6mm} \texttt{Tensor Lazy Red. Algorithm}

% \State Initialize: $\text{out} = A$
% \State \textbf{for} {$i = L$ \textbf{to} $2L+3$}  \hfill $\triangleright$ Higher $L$ Bytes, Reduce $B$
% \State \quad $\text{out} = \text{out} + x[8i+7: 8i] \cdot 256^i \bmod q$
% \State \textbf{Return} $\text{out}$ \hfill $\triangleright$  $L+2$ Bytes, Partially Reduced

% \hfill

% \noindent \hspace{-6mm} \texttt{TPU Implementation of Tensor Lazy Red.}
% \hfill

% \noindent \hspace{-4mm} \texttt{Offline} \hfill $\triangleright$  Precompute Reduction Coefficients
% \State $r_i = 256^{i+L} \bmod q, i\in[0,L+3]$ \hfill 
% \State $R_{i,j} = r_i[8j+7:8j], j\in[0,L-1]$ \hfill 
% \hfill \\
% \hfill

% \noindent \hspace{-4mm} \texttt{Online} \hfill $\triangleright$  Reduce High Part for a Batch of $b$ values
% \State $B_{idx,i}=x_{idx}[8i+7:8i], idx\in[0,b-1], i\in[L,2L+3]$
% \State return $B_{idx,i}@R_{i,j} + A_{idx,j} $ \hfill $\triangleright$  uint8 $b\cdot(L+4)\cdot L$ MatMul
% \end{algorithmic}
% \end{algorithm}

% \subsection{Detailed Explanation of Alg. \ref{alg:HP_on_LP_special_new}}
% \textbf{Chunk Decomposition:} Assuming the bit precision of hardware MAC is $bp$, a given data $a$ with $\log q$ bits will be broken down into $K=\lceil \frac{\log q}{bp} \rceil$ chunks $a^{k}$, $0\leq k< K$, each chunk has $bp$ bits, as shown in Alg.~\ref{alg:HP_on_LP_special_new}. All high-precision data will be stored and computed as chunks.

% \textbf{High-precision Scalar Addition:} A $\log q$-bit addition boils down to (1) chunk decomposition, (2) chunk-wise addition, (3) carry propagation across chunks, and (4) bitwise concatenation to merge chunks back to the high-precision result. 
% \THH{The algorithm for \textproc{HPScalarAdd} in~\algref{alg:HP_on_LP_special_new} doesn't match the description here. Line~\ref{alg:HP_on_LP_special_new:accum1} stills use high-precision addition for accumulation.}\JT{Resolved.}

% \textbf{High-precision Scalar Multiplication:} Multiplying two $\log q$-bit coefficients $a \times b$ to obtain a $2\log q$-bit result is mapped through (1) performing $K^2$ $bp$-bit multiplications for $a^i, b^j, (0\leq i,j< K)$, (2) shifted accumulation of chunk-wise multiplication results into final $2\log q$-bit result. 
% \THH{Like \textproc{HPScalarAdd}, Line~\ref{alg:HP_on_LP_special_new:accum2} stills use high-precision addition for accumulation.}\JT{Resolved.}


% \textbf{High-precision Shifted Scalar Multiplication:} 
% In Alg.~\ref{alg:barrett}, multiplying a \(\log q\)-bit number by a \(2\log q\)-bit number produces a \(3\log q\)-bit result, which is ultimately right-shifted by \(2\log q\) bits to yield a \(\log q\)-bit output. Therefore, the least significant \(2\log q\) bits serve only as temporary storage and need not be stored. To exploit this, \compiler partitions the \(2\log q\)-bit right shift into multiple steps, each discarding lower \(bp\) bits of the final result while accumulating chunk-wise multiplication product. As a result, this reduces $3\log q$-bit memory overhead of the final result to $\log q$ bits (Alg.~\ref{alg:HP_on_LP_special_new}).

% Operations in Alg.~\ref{alg:HP_on_LP_special_new} are only mapped to the VPU of TPUv4, which supports at most 32-bit integer arithmetic, i.e. $bp\leq32$. Mapping Alg.~\ref{alg:HP_on_LP_special_new} to MXU is inefficient because computation patterns does not fit the datapath of matrix multiplication engine, resulting in low utilization.

% These converted high-precision multiplication would then be converted into low-precision matrix multiplication following BAT detailed in Alg.~\ref{alg:HP_on_LP_special_new}.

% \begin{algorithm}
% \caption{Chunk Decomposition: Map High-precision Scalar Operations as Low-precision Chunk-wise Operations} \label{alg:HP_on_LP_special_new}
% \begin{algorithmic}[1]
% % \setlength{\algorithmicindent}{-3mm}
%  % \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%  % \renewcommand{\algorithmicensure}{\textbf{Output:}}
% % \algrenewcommand{\algorithmiccomment}[1]{\hskip-3em #1}
% % \setlength{\itemindent}{-3mm}
% % \setlength{\algorithmicindent}{-3mm}
% % \setlength{\itemindent}{-5mm}
% \Require $a,b,c \in \mathbb{Z}_{q}$ with \textbf{$\log q$}, \textbf{$\log q$}, \textbf{$2\log q$} bits, hardware bit precision $bp$, right shift $s$ bits for shifted mul.
% \State $K \leftarrow \lceil \frac{\log q}{bp}\rceil$  \hfill $\triangleright$ Number of chunks
% \Statex
% \Procedure{ChunkDecompose}{$a$}{} $\rightarrow \left[a^{k}\right]_{0\le k < K}$ 
% % \State  \textit{\textbf{--\hfill ChunkDecomposition$(a)$  $\rightarrow \left( a^{k}, k \in \left[0, \lceil \frac{logq}{bp}\rceil -1 \right] \right)$ \hfill--}}  
% % \State  $a^{k}\leftarrow $ bit range $\left[k\cdot bp, (k\+1)\cdot bp \right]$ of $a$, $0 \leq k < \lceil \frac{logq}{bp} \rceil$
% \State bits $\leftarrow$ binary($a$)
% \State  $a^{k}\leftarrow $ bits$\left[k\cdot bp: (k+1)\cdot bp \right]$, for $0 \leq k < K$
% \EndProcedure
% \Statex
% \Procedure{ChunkMerge}{$\left[a^{k}\right]_{0\le k < K}$}{} $\rightarrow a$
% % \State  \textit{\textbf{--\hfill ChunkDecomposition$(a)$  $\rightarrow \left( a^{k}, k \in \left[0, \lceil \frac{logq}{bp}\rceil -1 \right] \right)$ \hfill--}}  
% % \State  $a^{k}\leftarrow $ bit range $\left[k\cdot bp, (k\+1)\cdot bp \right]$ of $a$, $0 \leq k < \lceil \frac{logq}{bp} \rceil$
% \State  $a\left[k\cdot bp: (k+1)\cdot bp \right] = a^k$, for $0 \leq k < K-1$
% \EndProcedure
% \Statex
% \Procedure{CarryPropagate}{$\left[a^{k_1}\right]_{0\le k_1 < K}$}{} $\rightarrow$ $\left[z^{k_2}\right]$ $_{0\le k_2 < K+1}$  \hfill $\triangleright$ $z$ has $bp$ bits, $a$ has larger than $bp$ bits
% \State \textbf{for} iter in $K$:
% \State \quad $bits^{k}$ $\leftarrow$ binary($a^{k}$); $numbit^{k} \leftarrow len(bits^{k})$
% \State \quad $a_L^{k}$ $\leftarrow$ $numbit^{k}[0:numbit^{k} \gg -1]$; 
% \State \quad $a_H^{k}$ $\leftarrow$ $bits^{k}[numbit^{k} \gg:numbit^{k}-1]$
% \State \quad $z^{0} = a_L^{0}$; $z^{K} = a_H^{K}$; $z^{k} = a_L^{k+1} + a_H^{k}, 0< k < K$
% \State \quad $a^{k}=z^{k}$
% \EndProcedure
% \Statex
% \Procedure{HPScalarAdd}{$a, b$} $\rightarrow z $  \hfill $\triangleright$ $z=a+b$
% \State $\left[a^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$a$}
% \State $\left[b^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$b$}
% \State  $c^{k} = (a^{k} + b^{k})$, for $0 \leq k < K$ \label{alg:HP_on_LP_special_new:accum1} % \ll (k\cdot bp)$, 
% \State $z^{k} \leftarrow$ \Call{CarryPropagation}{$c^{k}$}, for $0 \leq k < K$ 
% \State $z \leftarrow $\Call{ChunkMerge}{$z^{k}$}, for $0 \leq k < K$
% \EndProcedure

% \Statex
% \Procedure{HPScalarMult}{$a, b$} $\rightarrow z$  \hfill $\triangleright$ $z=a \times b$
% \State $\left[a^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$a$}
% \State $\left[b^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$b$}
% \State  $c^{k_1+k_2} \mathrel{+}= \left(a^{k_1} \times b^{k_2}\right) \cdot bp$, for $0 \leq k_1, k_2 < K$\label{alg:HP_on_LP_special_new:accum2} %$\ll \left(k_1+k_2\right)$
% \State $z^{k} \leftarrow$ \Call{CarryPropagation}{$c^{k}$}, for $0 \leq k < 2K$ 
% \State $z \leftarrow $\Call{ChunkMerge}{$z^{k}$}, for $0 \leq k < 2K$
% % \mathrel{+}
% \EndProcedure

% \Statex
% \Procedure{HPShiftedMult}{$a,c$} $\rightarrow z$  \hfill $\triangleright$ $z=a\times c \gg s$
% \State $a^k, c^k \leftarrow$ \Call{ChunkDecompose}{$a,c$}
% \State $k_r = 0$ ($k_r$ records the total number of right shifting) 
% \State  \textbf{for} {$0 \leq k_z < \lceil \frac{3\log q}{bp}\rceil$}
% \State \quad \textbf{for} {$0 \leq k_1 \leq k_z$} 
% % \FOR {$0 \leq k_2 \leq \frac{logq}{bp}$}
% \State \quad \quad $z\ \+= \left(a^{k_1} \times c^{k_z - k_1}\right) \ll \left(k_z - k_r\right) \cdot bp$ 
% % \ENDFOR
% % \ENDFOR
% \State \quad \textbf{if} $ k_z < \lceil \frac{2\log q}{bp} \rceil$
% \State  \quad \quad $z = z \gg bp$  \hfill $\triangleright$ $z$ is always using $\log q$ bits
% \State \quad \quad $k_r\+\+$
% % \ENDIF
% % \ENDFOR
% \EndProcedure

% \end{algorithmic}
% \end{algorithm}


\begin{comment}
\subsection{Quantative NTT Throughput Comparison among SoTAs}
We compare the NTT throughputs among CROSS, HEAX, TensorFHE and FAB under various degree in \tabref{tab:ntt_throughput}~\cite{heax,agrawal2022fab,fan2022tensorfhe}, which shows that CROSS enable various generations of TPU to achieve the highest NTT throughput among existing publicly available devices.

\begin{table}[!htp]\centering
\caption{NTT throughput per second. The busy time ratio denotes the fraction of total latency during which the compute unit is active, not its actual compute utilization.}\label{tab:ntt_throughput}
%\resizebox{ extwidth}{!}{ % use this if the table is too large
\begin{tabular}{ccccc}\hline
uint: \#NTT/s &\textbf{Set A} &\textbf{Set B} &\textbf{Set C} \\\hline
Degree &$2^{12}$ &$2^{13}$ &$2^{14}$ \\
$log(Q)$ &109 &218 &438 \\ \hdashline
\rowcolor[gray]{0.9}\textbf{HEAX} &\textbf{195313} &\textbf{90114} &\textbf{41853} \\
\rowcolor[gray]{0.9}\textbf{TensorFHE} &\textbf{910134} &\textbf{449974} &\textbf{209337} \\ 
\rowcolor[gray]{0.9}\textbf{FAB} &  &  &\textbf{166156} \\ \hdashline
\rowcolor[HTML]{E6EFDB}\textbf{CROSS (TPUv6)} &\textbf{3330887} &\textbf{1664057} &\textbf{945020} \\
Best Batch Size &256 &128 &256 \\
VPU busy time ratio &{67.06}\% &{67.16}\% &{63.30}\% \\
MXU busy time ratio &{4.57}\% &{4.57}\% &{6.93}\% \\
Over HEAX &\textbf{17.05$\times$} &\textbf{18.47$\times$} &\textbf{22.58$\times$} \\
Over TensorFHE &\textbf{3.66$\times$} &\textbf{3.70$\times$} &\textbf{4.51$\times$} \\\hdashline
\rowcolor[HTML]{E6EFDB}\textbf{CROSS (TPUv5p) }&\textbf{4349471} &\textbf{2170446} &\textbf{1057909} \\
Best Batch Size &131072 &65536 &32768 \\
VPU busy time ratio &41.85\% &42.83\% &44.29\% \\
MXU busy time ratio &9.54\% &11.47\% &18.49\% \\
Over HEAX &\textbf{22.27$\times$} &\textbf{24.09$\times$} &\textbf{25.28$\times$} \\
Over TensorFHE &\textbf{4.78$\times$} &\textbf{4.82$\times$} &\textbf{5.05$\times$} \\ \hdashline
\rowcolor[HTML]{E6EFDB}\textbf{CROSS (TPUv5e)} &\textbf{2250568} &\textbf{1074241} &\textbf{530582} \\
Best Batch Size &128 &512 &256 \\
VPU busy time ratio &57.16\% &57.16\% &48.99\% \\
MXU busy time ratio &9.24\% &13.88\% &18.17\% \\
Over HEAX &\textbf{11.52$\times$} &\textbf{11.92$\times$} &\textbf{12.68$\times$} \\
Over TensorFHE &\textbf{2.47$\times$} &\textbf{2.39$\times$} &\textbf{2.53$\times$} \\ \hdashline
\rowcolor[HTML]{E6EFDB}\textbf{CROSS (TPUv4)} &\textbf{1367390} &\textbf{664757} &\textbf{311026} \\
Best Batch Size &2048 &1024 &256 \\
VPU busy time ratio &81.96\% &83.40\% &74.28\% \\
MXU busy time ratio &8.78\% &12.44\% &15.12\% \\
Over HEAX &\textbf{7.00$\times$} &\textbf{7.38$\times$} &\textbf{7.43$\times$} \\
Over TensorFHE &\textbf{1.50$\times$} &\textbf{1.48$\times$} &\textbf{1.49$\times$} \\
\hline
\end{tabular}
\end{table}
\end{comment}

% \begin{table}[!htp]\centering
% \caption{NTT/s (CROSS vs. FAB, $N=2^{14}, log2(Q)=438$)}\label{tab:vs_fab}
% %\resizebox{ extwidth}{!}{ % use this if the table is too large
% \begin{tabular}{cccccc}\hline
% & FAB &TPUv4 &TPUv5e &TPUv6 &TPUv5p \\\hline
% NTT/s & 166156.41 &311026 &530582 &945020 &1057909 \\
% Speedup & 1 &\textbf{1.87$\times$} &\textbf{3.19$\times$} &\textbf{5.69$\times$} &\textbf{6.37$\times$} \\
% \hline
% \end{tabular}
% \end{table}

% \begin{algorithm}
% \caption{CROSS Dedicated Mapping for 28-bit Modulus} \label{alg:HP_on_LP_special_new_special}
% \begin{algorithmic}[1]
% \Require modulus $q$ of $\log q$ bits, $a,b,c \in \mathbb{Z}_{q}$ with \textbf{$\log q$}, \textbf{$\log q$}, \textbf{$2\log q$} bits, hardware bit precision $bp$
% \State $K \leftarrow \lceil \frac{\log q}{bp}\rceil$ \hfill $\triangleright$ {Number of chunks (4 in our configuration)}
% \Statex
% \Procedure{BAT}{$b$} $\rightarrow \hat{b}^j_i$   \hfill $\triangleright$ offline compilation
% \State $\left[b^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$b$}
% \State   \hfill $\triangleright$ 1D-\textproc{im2col} converts $\left[b^k\right]$ into a matrix
% \State $\left[h_{ij}\right]_{\substack{0\le i < K\hfill\\ 0\le j < 2K-1}}\leftarrow$\Call{im2col}{$\left[b^k\right]$, kernel\_size=$(K,)$}
% \State $\hat{b}^j_i \leftarrow h_{ij}$ \textbf{for} $0\le i,j<K$
% \For {$0 \le i < K$}
%     \State $c_i \leftarrow 0$
%     \For {$K \le j < 2K-1$}
%         \State $c_i \mathrel{+}= h_{ij}*2^{bp(i+j-K)}$
%     \EndFor 
%     \State \algorithmicdo   \hfill $\triangleright$ redistribute chunks of higher bases
%         \State \quad $c_i \mathrel{*}= 2^{bp*K}$
%         \State \quad $\left[c^k\right]_{0\le k <K} \leftarrow$ \Call{ChunkDecompose}{$c_i\mod q$}
%         \State \quad $\left[\hat{b}^k_i\right]_{0\le k <K} \mathrel{+}= [c^k]_{0\le k < K}$
%         \State \quad $\left[\hat{b}^k_i\right]_{0\le k < K},c_i$ $\leftarrow$ \Call{CarryPropagate}{$\left[\hat{b}^k_i\right]_{0\le k < K}$}
%     \State \algorithmicwhile \quad {$c_i \neq 0$}
% \EndFor
% % \State {bottom K-1}
% % \State $\left[b^j_i\right]_{0\le i,j < K} \leftarrow$ \Call{BAT}{$b$}
% % \State $\left[c^{i}\right]_{0 \le i < K}$ = \Call{BAT}{$\left[a^k\right]_{0\le k < K}$ ,$\left[b^j_i\right]_{0\le i,j < K}$}
% % \State $z \mathrel{+}= c^{i} \ll 8^i, 0 \le i < K$
% \EndProcedure
% \Statex
% \Procedure{HPScalarMult-BAT}{$a, b$} $\rightarrow z$ 
% \State $\left[a^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$a$}
% \State $\left[\hat{b}^j_i\right]_{0\le i,j < K} \leftarrow$ \Call{BAT}{$b$}
% \State $\left[c^{j}\right]_{0 \le j < K}$ = $\left[\hat{b}^j_i\right]_{0\le i,j < K} \times \left[a^j\right]_{0\le j < K}$ 
% \State $z \mathrel{+}= c^{j} \ll (bp*j), 0 \le j < K$
% \EndProcedure
% \Statex
% \Procedure{HPScalarMult-Conv}{$a, b$} $\rightarrow z$ 
% \State $\left[a^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$a$}
% \State $\left[b^k\right]_{0\le k < K} \leftarrow$ \Call{ChunkDecompose}{$b$}
% \State $\left[c^{i}\right]_{0 \le i < 2K-1}$ = \Call{1DConv}{$\left[a^k\right]_{0\le k < K}$ ,$\left[b^k\right]_{0\le k < K}$}
% \State $z \mathrel{+}= c^{i} \ll (bp*i)$ for $0 \le i < 2K-1$
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

==> src/rebuttal.tex <==


\researchquestionA{\textbf{RA-Q1}: \textbf CROSS on CPUs with matrix math (e.g. Intel's AMX /AVX or ARM's SME)?}
We extend CROSS to CPUs supporting AVX (tested on AMD 9950X3D), achieving\textbf{ 16.8$\times$ latency speedup} on HE kernels, as shown in \tabref{tab:perf_cmp_cpu} and discussed in \secref{q:ra_q1}.

\researchquestionA{\textbf{RA-C2}: Terminology in Alg. \autoref{alg:HP_on_LP_special_new} needs explanation}
We enhance Alg. \autoref{alg:HP_on_LP_special_new} with explanation and link to \figref{fig:CROSS_Scalar_Flow}.


\researchquestionC{\textbf{RC-C2}: Why not unify metrics for NTT and HE kernels?} %Throughput comparison for BConv, bootstrapping, AutoMorph, VecModAdd, VecModMul and LR?
We adopt metrics from prior work for consistency of apple-to-apple comparison: throughput for NTT \cite{heax,fan2022tensorfhe} and latency for HE kernels/ML workloads, (clarify in \secref{q:rc_c2}/\textbf{Metrics}).

\researchquestionC{\textbf{RC-C3}: Authors provide details on parameter set}
We now include full parameter configurations in \secref{q:rc_c3}. CROSS adopts the default TPU parameters in \tabref{tab:perf_cmp} ($logq<32$, $N=2^{16}$, $L=51$, $dnum=3$ which shows high TPU’s compute utilization and less on-chip memory reorganization.

\researchquestionC{\textbf{RC-C4}: How to calculate the speedup in \tabref{tab:perf_cmp}?} Energy-efficiency improvement is defined as the latency ratio of prior work to CROSS, normalized by power ratio. Values $<1$ indicate lower efficiency than ASICs. We highlight CROSS’s wins with $\uparrow$ and clarify this in \tabref{tab:perf_cmp}’s caption.

\researchquestionD{\textbf{RD-C1,C4}: Move acknowledge earlier, Reform evaluation organization, give key takeaways}

We reform evaluation section and summarize \textbf{\textit{Takeaway}}. 

\researchquestionD{\textbf{RD-C2}: Evidence for SoTA GPU being 10$\times$ less energy efficient than HE ASIC in introduction} 
We added references in \secref{q:rd_c2}, explaining both architectural reasons for this gap, and linked to supporting data in \tabref{tab:perf_cmp}.

\researchquestionD{\textbf{RC-C5, RD-C4}: Inconsistent generations of TPU}

\noindent \textbf{Energy efficiency} experiment only uses TPUv4 (170 W TDP \cite{jouppi2023tpu}) as other TPUs' data are not publicly available. \textbf{Latency results} include all TPU generations. Clarified in \secref{q:rc_c5}.

\researchquestionE{\textbf{RE-Q1}: Can CROSS maintain performance advantage and correctness for e2e ML workload?}
Yes. CROSS's verified against OpenFHE to generate same results under identical input and parameters, achieving 98\% accuracy and 49 ms latency for LoLa-MNIST on TPUv4, as detailed in \secref{q:re_q1}.

\researchquestionE{\textbf{RE-Q2}: Are CROSS results bitwise identical to full-precision HE algorithms?}
Yes. CROSS optimizations (BAT and MAT) are\textbf{ lossless transformations }that restructure computation without losing precision, as clarified in \secref{q:re_q2}.


\researchquestionE{\textbf{RE-C1}: implementations of carry add (multi-chunk reduction)?} 
Carry addition is performed in the VPU using 32-bit arithmetic. chunks are accumulated into 64-bit integers, and get stored as two 32-bit chunks. We clarify it in \secref{q:re_c1}.

\researchquestionE{\textbf{RE-C2}: implementations of lazy reduction?}

Lazy reduction refers to the \textbf{Montgomery reduction }(Alg. \autoref{alg:montgomery_reduction}), where intermediate values may temporarily exceed $q$ without immediate reduction (hence call it lazy). We clarify it in \figref{fig:CROSS_Scalar_Flow} and its caption.


\researchquestionF{\textbf{RF-Q1}: Results of CROSS under consistent parameters?}
We add single-batch HE-kernel latency under same parameters as prior works, with detailed bottleneck analysis in \secref{q:rf_q1}.

\researchquestionF{\textbf{RF-Q2}: TPUv4's bootstrapping latency?}
Measured at \textbf{1230} µs, now listed in \tabref{tab:bootstraping}.

\researchquestionF{\textbf{RF-Q3/C4}: Performance of different reduction algorithms?}

We evaluate Barrett, Montgomery, and Shoup reductions for (1) VecModMul and (2) NTT. Results show NTT favors Montgomery + BAT, while Shoup slightly outperforms others in VecModMul, as shown in new \figref{fig:diff_modred} and new \secref{q:rf_q3}.


\researchquestionF{\textbf{RF-Q4}: Why is (H, V, W) = (512, 1024, 1024) result far from expected speedup (1.1$\times$ vs. 2$\times$)?}
The BAT-transformed matrix multiplication consists of three stages: (1) \textbf{bitcast}: decomposing each 32-bit value into four 8-bit chunks, (2) \textbf{low-precision GEMM} (in BAT) or convolution (in baseline), and (3) \textbf{partial-sum accumulation}, as illustrated in \figref{fig:CROSS_Scalar_Flow}. BAT yields average latency reductions of 2.0$\times$, 1.6$\times$, and 1.6$\times$ across these stages. The limited overall gain (1.1$\times$ vs. 2$\times$ expected) primarily arises from host–device synchronization overhead, where the TPU stalls waiting for CPU scheduling decisions imposed by the XLA runtime. Further details are clarified in \secref{q:rf_q4}.

\researchquestionF{\textbf{RF-C1}: results for LoLa-MNIST}

Results are discussed in \secref{q:re_q1}. Since prior works lack latency/accuracy data for LoLa-MNIST, we compare CROSS only against CPU baselines without adding a table.

\researchquestionF{\textbf{RF-C3}: details reasons for 2$\sim$3$\times$ performance penalty for special modulus.}
Dedicated ASICs can hard-wire compute-friendly moduli such as $q = 2^{32} - v$ (with small $v$), eliminating runtime parameter broadcasting. This design halves memory traffic for each vectorized multiplication between operands and $v$, yielding up to 2$\times$ speedup for memory-bound arithmetic. The additional saving from removing constant broadcasts and instruction overhead further increases the advantage to 2$\sim$3$\times$.


\researchquestionF{\textbf{RF-C5}: Add architectural comparison CPU/GPU/FPGA}
We include \tabref{tab:arch_high_lvl_diff}, summarizing differences in clock frequency, on-chip memory, programmability, and throughput.

\researchquestionF{\textbf{RF-C6}: why is a apple-to-apple comparison to other works using different modular reduction schemes?} 
It's fair as each platform uses its best-performing under given accuracy requirement ($<1$ \% accuracy loss vs. unencrypted baseline). Clarified in \tabref{tab:perf_cmp}’s caption.

% \thispagestyle{firstpage}
\pagestyle{plain}
\newpage
